Paschke Dilations

In 1973 Paschke defined a factorization for completely positive maps between C*-algebras. In this paper we show that for normal maps between von Neumann algebras, this factorization has a universal property, and coincides with Stinespring's dilation for normal maps into B(H).

==> eptcsdata.tex <==
\providecommand{\firstpage}{229}
\providecommand{\publicationstatus}{R. Duncan and C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2016\\
EPTCS 236, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.236.15}{10.4204/EPTCS.236.15}}
\pdfoutput=1

